InsertionNet 2.0: Minimal Contact Multi-Step Insertion Using Multimodal Multiview Sensory Input

We address the problem of devising the means for a robot to rapidly and safely learn insertion skills with just a few human interventions and without hand-crafted rewards or demonstrations. Our InsertionNet version 2.0 provides an improved technique to robustly cope with a wide range of use-cases featuring different shapes, colors, initial poses, etc. In particular, we present a regression-based method based on multimodal input from stereo perception and force, augmented with contrastive learning for the efficient learning of valuable features. In addition, we introduce a one-shot learning technique for insertion, which relies on a relation network scheme to better exploit the collected data and to support multi-step insertion tasks. Our method improves on the results obtained with the original InsertionNet, achieving an almost perfect score (above 97.5$\%$ on 200 trials) in 16 real-life insertion tasks while minimizing the execution time and contact during insertion. We further demonstrate our method's ability to tackle a real-life 3-step insertion task and perfectly solve an unseen insertion task without learning.

==> task_description.tex <==
\section{TASK DESCRIPTION}
\label{sec:GeneralInsertion}
Our primary objective in this work is to develop an algorithm that is directly applicable to as many real-world insertion tasks as possible. In this section, we elaborate on what a \emph{general insertion solution} means. \\
\textbf{Scalability:} A general solution should be able scale to different peg-in-a-hole, plug insertion, and threading problems, etc. The solution should be able to simultaneously solve all these use-cases with a single pre-trained policy. \\
\textbf{Minimal Contact:} Contact with the hole surface during insertion may damage the product and increase the insertion time. Policy should minimize the contact with the environment.
\textbf{Size Independence:} The peg and the hole size can vary between different assembly applications, from avionic to micro-electronic products. A general algorithm should not be size dependent. \\
\textbf{Unfixed Grasping:}  In many of the currently available solutions, the grasping aspect of the problem is ignored by fixing the plug to the EEF. In our case, accidental peg slips and limited manipulation is considered and learned. \\
\textbf{Location:} The ability to insert the same peg repeatedly in different locations is necessary in many industrial applications, such as electrical panel assembly. Therefore, it is required that an algorithm operate in any given location or orientation without additional learning. \\
\textbf{Transfer Learning Capabilities:} The algorithm should be able to share information between different insertion tasks. Therefore, training a new insertion task should require less data than learning the task from scratch.
